SRWarp: Generalized Image Super-Resolution under Arbitrary Transformation

Deep CNNs have achieved significant successes in image processing and its applications, including single image super-resolution (SR). However, conventional methods still resort to some predetermined integer scaling factors, e.g., x2 or x4. Thus, they are difficult to be applied when arbitrary target resolutions are required. Recent approaches extend the scope to real-valued upsampling factors, even with varying aspect ratios to handle the limitation. In this paper, we propose the SRWarp framework to further generalize the SR tasks toward an arbitrary image transformation. We interpret the traditional image warping task, specifically when the input is enlarged, as a spatially-varying SR problem. We also propose several novel formulations, including the adaptive warping layer and multiscale blending, to reconstruct visually favorable results in the transformation process. Compared with previous methods, we do not constrain the SR model on a regular grid but allow numerous possible deformations for flexible and diverse image editing. Extensive experiments and ablation studies justify the necessity and demonstrate the advantage of the proposed SRWarp method under various transformations.

==> figs/teaser_submission.tex <==
\begin{figure}[t]
    \centering
    %\addtocounter{subfigure}{-1}
    \subfloat[Projective transform]{\includegraphics[width=0.49\linewidth]{figs/div2k_0600/teaser.png}}
    \hfill
    \subfloat[OpenCV]{\includegraphics[width=0.245\linewidth]{figs/div2k_0600/1_cv2.png}}
    \hfill
    \subfloat[\textbf{SRWarp}]{\includegraphics[width=0.245\linewidth]{figs/div2k_0600/1_proposed.png}}
    \\
    \figcspace
    \caption{
        \textbf{Image transformation with the proposed SRWarp.}
        %
        Our method can reconstruct HR images of arbitrary shapes and resolutions from a given LR input without noticeable artifacts and aliasing.
    }
    \label{fig:teaser}
    \figspace
\end{figure}

==> submission/0_abstract.tex <==
\begin{abstract}
    Deep convolutional neural networks (CNNs) have achieved significant successes in image processing and its applications, including single-image super-resolution (SR).
    %
    However, the conventional methods still resort to some predetermined integer scaling factors, e.g., $\times 2$ or $\times 4$, and it is difficult to apply such SR algorithms when arbitrary target resolutions are required.
    %
    Recent approaches extend the scope to fractional upsampling factors, even with varying aspect ratios to handle the limitation.
    %
    In this paper, we propose the SRWarp framework to further generalize the SR tasks toward an arbitrary image transformation.
    %
    We interpret the traditional image warping task, specifically when the input is enlarged, as a spatially-varying SR problem.
    %
    We also propose several novel formulations, including the adaptive warping layer and multi-scale blending, to reconstruct visually favorable results in the transformation process.
    %
    Compared to previous methods, we do not constrain the SR model on a regular grid but allows numerous possible deformations for flexible and diverse image editing.
    %
    Extensive experiments and ablation studies justify the necessity and demonstrate the advantage of the proposed SRWarp method under various transformations.
\end{abstract}

==> submission/1_intro.tex <==
\section{Introduction}
%
Single-image super-resolution~(SISR or SR) is one of the fundamental vision problems which aims to reconstruct a high-resolution~(HR) image from a given low-resolution~(LR) input.
%
Due to its practical importance, the SR methods are widely used in image processing applications such as perceptual image enhancement~\cite{sr_srgan, sr_esrgan}, editing~\cite{sr_explorable, sr_srflow}, and digital zooming~\cite{wronski2019handheld}.
%
Just like the other vision-related tasks, recent deep neural networks have achieved promising SR performances with large-scale datasets~\cite{data_div2k, sr_edsr}, efficient structures~\cite{sr_rcan, sr_rdn, sr_dbpn}, and novel optimization techniques~\cite{sr_edsr, sr_esrgan}.
%
Recent state-of-the-art methods can reconstruct sharp edges and crisp textures with fine details up to $\times 4$ or $\times 8$ scaling factors on various types of input data including real-world images~\cite{sr_zllz, sr_realworld, sr_cdc}, videos~\cite{vsr_edvr, vsr_zooming_slowmo, vsr_starnet, vsr_tdan, vsr_mucan}, hyperspectral~\cite{Fu_2019_CVPR, Zhang_2020_CVPR, yao2020cross}, and light field arrays~\cite{Zhang_2019_CVPR, sr_crossnetpp, wang2020spatial}.


From the perspective of image editing applications, the SR algorithm supports users to effectively increase the number of pixels in the image and reconstruct high-frequency details when its HR counterpart is not available.
%
Such manipulation may include simple resizing with some predefined scaling factors or synthesizing images of arbitrary target resolutions.
%
However, it is not easy to apply existing SR methods in those situations directly since the models are usually designed to cope with some fixed integer scales~\cite{sr_srgan, sr_rcan, sr_esrgan}.
%
Recently, few methods have extended the scope of the SR to upsample a given image by arbitrary scaling factors~\cite{sr_meta} and aspect ratios~\cite{sr_arb}.
%
Those novel approaches provide more flexibility and versatility to existing SR applications for their practical usage.

\begin{figure}[t]
    \centering
    %\addtocounter{subfigure}{-1}
    \subfloat[Projective transform]{\includegraphics[width=0.49\linewidth]{figs/div2k_0600/teaser.png}}
    \hfill
    \subfloat[OpenCV]{\includegraphics[width=0.245\linewidth]{figs/div2k_0600/1_cv2.png}}
    \hfill
    \subfloat[\textbf{SRWarp}]{\includegraphics[width=0.245\linewidth]{figs/div2k_0600/1_proposed.png}}
    \\
    \figcspace
    \caption{
        \textbf{Image transformation with the proposed SRWarp.}
        %
        Our method can reconstruct HR images of arbitrary shapes and resolutions from a given LR input without noticeable artifacts and aliasing.
    }
    \label{fig:teaser}
    \figspace
\end{figure}

Nevertheless, existing SR models are not fully optimized for general image editing tasks due to their intrinsic formulations.
%
As digital images are defined on a rectangular grid, previous approaches are also designed to take and reconstruct such rectangular frames.
%
In contrast, images may undergo various deformations in practice so that their contents can be adjusted well within context.
%
For instance, homographic transformation~\cite{zhang2020content, le2020deep} aligns images from different views, and cameras incorporate various correction algorithms to remove distortions from the lens~\cite{swaminathan2000nonmetric, xue2019learning}.
%
One of the shortcomings in the conventional warping methods is that interpolation-based algorithms tend to generate blurry results when a local region of the image is stretched.
%
Hence, an appropriate enhancement algorithm is required to preserve sharp edges and detailed textures, as the SR methods for image upscaling.
%
However, such applications may require images to be processed on irregular grids, which cannot be handled by na\"ive CNNs for regular-shaped data.


To prevent blurry warping results, it is possible to introduce a state-of-the-art SR model prior to the image transformation.
%
By doing so, supersampled pixels may alleviate blurriness and artifacts from simple interpolation.
%
While such an approach can dramatically improve the quality of image transformation, Hu~\etal~\cite{sr_meta} and Wang~\etal~\cite{sr_arb} have already demonstrated that the solution is suboptimal in the case of the arbitrary-scale SR task.
%
Furthermore, a generalized warping algorithm has to deal with more complex and even spatially-varying deformations, which are not easy to be considered in the previous approaches.
%
%Therefore, it is not straightforward to simply combine the SR and warping methods, and a proper solution is required to optimize.
%
Therefore, a proper solution is required to effectively combine the SR and warping methods in a single pipeline.


We interpret the general image transformation task as a spatially-varying SR problem and propose an end-to-end learnable framework: SRWarp.
%
Unlike the previous SR methods, our model is designed to handle the warping problem in two specific aspects.
%
First, we introduce an adaptive warping layer to dynamically predict appropriate resampling kernels for different local distortions.
%
Second, our multi-scale blending strategy combines features of various resolutions based on their contents and local deformations to utilize richer information from a given image.
%
With powerful backbones~\cite{sr_edsr, sr_esrgan}, the proposed SRWarp can successfully reconstruct image structures that can be missed from conventional warping methods, as shown in \figref{fig:teaser}.
%
Our contributions can be summarized in threefolds:
%
\begin{compactitem}[$\bullet$]
    \item The novel SRWarp model generalizes the concept of SR under arbitrary transformations and formulates a framework to learn the image transformation.
    %
    \item Extensive analysis shows that our adaptive warping layer and multi-scale blending contribute to improving the proposed SRWarp method.
    %
    \item Our SRWarp model can reconstruct high-quality details and edges in transformed images compared to existing methods, both quantitatively and qualitatively.
\end{compactitem}

==> submission/2_related.tex <==
\section{Related Work}
\Paragraph{Conventional deep SR.}
%
After SRCNN~\cite{sr_srcnn} has successfully proved the potential of CNNs for the SR task, numerous methods have been developed toward better reconstruction.
%
The VDSR~\cite{sr_vdsr} model introduces a residual learning strategy to enable faster training and very deep network architecture, and the ESPCN~\cite{sr_espcn} model proposes a pixel-shuffling layer to implement a learnable upsampling module.
%
The LapSRN~\cite{sr_lapsrn} architecture efficiently handles the multi-scale SR task using a laplacian upscaling pyramid.
%
Ledig~\etal~\cite{sr_srgan} have adopted the residual block from high-level image classification task~\cite{net_residual} to implement SRResNet and SRGAN architectures.
%
With increasing computational resources, state-of-the-art methods such as the EDSR model~\cite{sr_edsr} have focused on larger and more complex network structures.
%
Several advances in recent SR methods such as attention~\cite{sr_rcan, sr_san, sr_han}, back-projection~\cite{sr_dbpn}, and dense connections~\cite{sr_rdn, ir_rdn, sr_dbpn, sr_esrgan}, making it possible to reconstruct high-quality images very efficiently.


\Paragraph{SR for arbitrary resolution.}
%
Before Shi~\etal~\cite{sr_espcn} have introduced the subpixel convolution for learnable upscaling, most of conventional SR methods~\cite{sr_srcnn, sr_vdsr} have relied on na\"ive interpolation to enlarge a given LR image.
%
For example, the VDSR~\cite{sr_vdsr} model upscale the LR image to their target resolution and then apply the SR model to refine local details and textures.
%
While the method can serve as an arbitrary-scale SR framework, a significant drawback is that extensive computations are required proportional to the output dimension.
%
Therefore, later methods have been specialized to some fixed scaling factors, e.g., $\times 2$ or $\times 4$, which are commonly used in various applications.


Recently, Hu~\etal~\cite{sr_meta} have proposed the meta-upscale module to replace scale-specific upsampling layers in previous approaches.
%
The Meta-SR model is designed to utilize dynamic filters concerning the target scale to deal with arbitrary upscaling factors. 
%
Later, Wang~\etal~\cite{sr_arb} introduce scale-aware convolution and upsampling modules to reconstruct images of arbitrary target resolutions.
%
While the previous methods mainly consider the SR task on horizontal or vertical axes, our differentiable warping module in SRWarp allows images to be transformed into any shapes.


\Paragraph{Irregular spatial sampling in CNNs.}
%
In a digital image, pixels are uniformly placed on a 2D rectangle.
%
However, objects in the image may appear in arbitrary shapes and orientations, making it challenging to handle them with a simple convolution operation.
%
To overcome the limitation, the spatial transformer networks~\cite{jaderberg2015spatial} estimate an appropriate warping parameter to compensate for possible deformations in the input image.
%
Rather than transform the image, deformable convolutions~\cite{dai2017deformable} and active convolutions~\cite{jeon2017active} predict input-dependent kernel offsets and modulation factors~\cite{zhu2019deformable} to perform irregular sampling from given features.
%
Furthermore, the deformable kernel~\cite{gao2019deformable} methods resample filter weights to adaptively adjust the effective receptive field during inference.
%
While several state-of-the-art image restoration models, especially with temporal data, introduce the irregular sampling strategy for accurately alignment~\cite{vsr_tdan, vsr_edvr, vsr_zooming_slowmo}, our approach is the first novel attempt to interpret the warping as an SR problem.

==> submission/3_method.tex <==
\section{Method}
%
We introduce our generalized SR framework, namely SRWarp, in detail.
%
Each of the term $\img{LR} \in \mathbb{R}^{H \times W}$, $\img{HR} \in \mathbb{R}^{H' \times W'}$, and $\img{SR} \in \mathbb{R}^{H' \times W'}$ represent source LR, ground-truth HR, and target super-resolved images, respectively.
%
$H \times W$ and $H' \times W'$ correspond to image resolutions, and we omit RGB color channels for simplicity.
%
Unlike the conventional SR task, the target resolution $H' \times W'$ varies depends on the transformation.
%
Since the warped sample may have irregular shapes rather than rectangular, we define its resolution using a bounding box of the image.


\subsection{Super-Resolution Under Homography}
\label{ssec:generalize}
%
Given a $3 \times 3$ projective homography matrix $M$ and a point $p = \paren{ x, y, 1 }\transpose$ on the source image, we calculate the target homogeneous coordinate $p' = w' \paren{ x', y', 1 }\transpose$ as $Mp = p'$ or $f_M \paren{ x, y } = \paren{ x', y' }$, where $f_M$ is a corresponding functional representation.
%
In the backward warping, $p = M^{-1} p'$ is calculated instead for each output pixel $p'$ to remove cavities.
%in the target image.
%
If we scale the image along $x$ and $y$-axis only, the matrix $M$ can be simplified as follows:
%
\begin{equation}
    M_{s_x s_y} =
    \begin{pmatrix}
        s_x & 0 & 0.5 \paren{ s_x - 1 } \\
        0 & s_y & 0.5 \paren{ s_y - 1 } \\
        0 & 0 & 1
    \end{pmatrix},
    \label{eq:scale_matrix}
\end{equation}
%
where $s_x$ and $s_y$ denote corresponding scale factors along the axes, and the translation components compensate subpixel shift to ensure an accurate alignment~\cite{opencv_library}.
%
Most of the early SR methods are designed to deal with the case where $s_x = s_y$ are some predefined integers~\cite{sr_espcn, sr_srgan, sr_dbpn, sr_esrgan}.
%
While recent approaches have relaxed such constraint by allowing arbitrary real numbers for $s_x$ and $s_y$~\cite{sr_meta, sr_arb}, numerous possible transformations $M$ are remaining unexplored.


\figref{fig:pyramid} presents a realization of conventional SR methods and our SRWarp approach from the perspective of the image scale pyramid.
%
For convenience, we assume that an LR image is placed on the plane $z = 1$.
%
Then, the $\times s$ SR result is equivalent to a slice of the pyramid by the plane $z = s$, where all points on the super-resolved image have the same $z$-coordinate.
%
Previous methods aim to learn the representations on the planes that are parallel to the given LR sample.
%
However, it is also possible to slice the image pyramid with an arbitrary plane, or even general surfaces, in the space.
%
Since the pixels in the resulting image can have different $z$ values depending on their positions, we propose to redefine the warping problem as a generalized SR task with spatially-varying scales and even aspect ratios.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/pyramid.pdf}
    \\
    \figcspace
    \caption{
        \textbf{Concept of the generalized SR.}
        %
        Dotted lines represent the upscale image pyramid in $xyz$-coordinate.
        %in $xyz$-coordinate.
        %
        While $\times s$ super-resolved images from conventional methods~(\textcolor{red}{\textbf{red}}) exist on the plane $z = s$ only, our results~(\textcolor{blue}{\textbf{blue}}) exists on any arbitrary cutting surfaces of the pyramid.
        %
        We note that the aspect ratio of the pyramid can be varied as well.
    }
    \label{fig:pyramid}
    \figspace
\end{figure}


\subsection{Adaptive Warping Layer}
\label{ssec:elliptical}
%
Image warping consists of two primitive functions: mapping and resampling.
%
%Given a target coordinate $p'$, the corresponding source pixel is located as $\round{ p }$, where $\round{ \cdot }$ is an element-wise rounding.
Given a target position $p' = \paren{ x', y' }$, the corresponding source pixel is determined as $p = \paren{ x, y }$, from a given transformation.
%
We omit the homogeneous representation for simplicity.
%
However, pixels in digital images are placed on integer coordinates only, making it infeasible to acquire a value from the position $p$ directly.
%
%The relationship between the points $p'$ and $p$ can be derived from a given mapping function, e.g., $p = M^{-1} p'$ in homographic transformation.
%
%This mapping operation is nonparametric and shared across conventional warping and our approach.
%
Therefore, an appropriate resampling or filtering process is required to reduce artifacts and ensure smoothness as follows:
%
%However, due to the mismatch between values at the subpixel $p$ and $\round{p}$ on the source domain, an appropriate resampling is required to reduce artifacts and ensure smoothness as follows:
%
\begin{equation}
    \mathbf{W} \paren{ x', y' } = \sum_{i, j = a}^{ b } { \mathbf{k} \paren{ x', y', i, j } \mathbf{F} \paren{ \round{x} + i, \round{y} + j } },
    \label{eq:kernel}
\end{equation}
%
where $\round{ \cdot }$ is a rounding operator, $\mathbf{F} \in \mathbb{R}^{H \times W}$ is an input, $\mathbf{W} \in \mathbb{R}^{H' \times W'}$ is an output, and $\mathbf{k}$ is an interpolation kernel centered around the point $\paren{ \round{x}, \round{y} }$, respectively.
%
$a$ and $b$ are boundary indices of a $k \times k$ window, where $k = b - a + 1$.
%
We set $a = -1$ and $b = 1$ with standard $3 \times 3$ kernels.


The traditional algorithm introduces a fixed sampling coordinate and kernel function to calculate the weight $\mathbf{k}$, regardless of the transformation $M$.
%
For example, a widely-used bicubic warping first calculates relative offset $\paren{ o_x, o_y }$ of each point in the window with respect to $\paren{x, y}$ as shown in \figref{fig:example_area_regular} and constructs $\mathbf{k}$ using a cubic spline.
%
However, due to the diversity of possible transformations, such formulation can be suboptimal in several aspects.
%
First, it is not easy to consider the transformed geometry where the target image is not defined on a rectangular grid.
%
Second, the interpolation tends to produce a blurry result as it takes a weighted average of neighboring values.
%
Also, the kernel function is fixed, while recent SR models prefer learnable upsampling methods~\cite{sr_espcn, sr_meta, sr_arb} rather than the predetermined one~\cite{sr_vdsr}.
%
To handle the issues mentioned above, we propose an adaptive warping layer (AWL) so that the resampling kernel $\mathbf{k}$ can be trained to consider local deformations.


\input{figs/kernel}


To determine a proper sampling coordinate for each target position $\paren{ x', y' }$, we first linearize the backward mapping $M^{-1}$ at the point with the Jacobian matrix $J \paren{ x', y' } = \begin{pmatrix} \mathbf{u}\transpose & \mathbf{v}\transpose \end{pmatrix}$, where $\mathbf{u}$ and $\mathbf{v}$ can be calculated as follows:
%
\begin{equation}
    \begin{split}
        \mathbf{u} &= \frac{f^{-1}_{M} \paren{ x' + \epsilon, y'} - f_{M}^{-1} \paren{ x' - \epsilon, y'}}{2 \epsilon}, \\
        \mathbf{v} &= \frac{f^{-1}_{M} \paren{ x', y' + \epsilon} - f^{-1}_{M} \paren{ x', y' - \epsilon}}{2 \epsilon}, \\
    \end{split}
    \label{eq:approximation}
\end{equation}
%
where $f^{-1}_{M} = f_{M^{-1}}$ and $\epsilon = 0.5$.
%
Using the local approximation, we project a unit circle centered around $\paren{ x', y' }$ on the target domain to an ellipse~\cite{ewa} on the source image.
%
Then, we redefine the resampling coordinate with two principal axes $\mathbf{e'}_x$ and $\mathbf{e'}_y$ of the ellipse.
%
By doing so, the relative offset $\paren{ o'_x, o'_y }$ of each point in the kernel window $\mathbf{k}$ can be adaptively adjusted depending on the local distortion as shown in \figref{fig:example_area_irregular}.


Next, we introduce a kernel estimator $\mathcal{K}$ to estimate proper resampling weights $\mathbf{k}$.
%
Similar to the conventional interpolation methods, the module takes $k^2$ offset vectors to determine contributions of each point $\mathbf{F} \paren{ x, y }$ in the window $\mathbf{k} \paren{ x', y' }$.
%
However, we introduce a series of fully-connected layers~\cite{sr_meta, sr_arb} so that the optimal kernel function can be learned from training data rather than predetermined.
%
Combining the adaptive resampling grid and differentiable kernel prediction layer $\mathcal{K}$, our AWL can consider local deformations and generate proper dynamic filters~\cite{jia2016dynamic, vsr_duf} for the given transformation.
%
The adaptive warping layer $\mathcal{W}$ is defined as follows:
%
\begin{equation}
    \mathbf{W} = \mathcal{W} \paren{ \mathbf{F}, f_{M} }.
    \label{eq:awl}
\end{equation}


\subsection{Multi-Scale Blending}
\label{ssec:ms_warping}
%
\figref{fig:pyramid} illustrates that images under the generalized SR task suffer distortions with spatially-varying scaling factors.
%
Therefore, multi-scale representations can play an essential role in reconstructing high-quality images.
%
To effectively utilize the property, we further introduce a blending method for the proposed SRWarp framework.


\Paragraph{Multi-scale feature extractor.}
%
We first define a scale-specific feature extractor $\mathcal{F}_{\times s}$ with a fixed integer scaling factor of $s$, which adopts the state-of-the-art SR architectures~\cite{sr_edsr, sr_esrgan}.
%
Given an LR image $\img{LR}$, the module extracts the scale-specific feature $\mathbf{F}_{\times s} \in \mathbb{R}^{C \times sH \times sW}$, where $C$ denotes the number of output channels.
%
While it is possible to separate the network for each scaling factor, we adopt a shared feature extractor with multiple upsampling layers~\cite{sr_edsr} in practice for several reasons.
%
For instance, previous approaches have demonstrated that multi-scale representations can be jointly learned~\cite{sr_vdsr, sr_lapsrn, lai2018fast, sr_arb} within a single model.
%
It is also computationally efficient to use the shared network rather than forwarding an input to multiple models for different scaling factors.
%
From the state-of-the-art SR architecture, we replace the last upsampling module with $\times 1$, $\times 2$, and $\times 4$ feature extractor to implement our multi-scale backbone as shown in \figref{fig:architecture}.


\Paragraph{Multi-scale warping and blending.}
%
For each scale-specific feature $\mathbf{F}_{\times s}$, we construct the corresponding transformation as $M M_{s^{-1} s^{-1}}$ using \eqref{eq:scale_matrix}.
%
By doing so, features of different resolutions can be mapped to a fixed spatial dimension, i.e., $H' \times W'$.
%
We use a term $\mathbf{W}_{\times s} \in \mathbb{R}^{C \times H' \times W'}$ to represent the warped features as follows:
%
\begin{equation}
    \mathbf{W}_{\times s} = \mathcal{W} \paren{ \mathcal{F}_{\times s} \paren{ \img{LR} }, MM_{s^{-1} s^{-1}} }.
    \label{eq:ms_warping}
\end{equation}
%
Then, the output super-resolved image $\img{SR}$ can be reconstructed from a set of the multi-scale warped features $\left\{ \mathbf{W}_{\times s} | s = s_0, s_1, \cdots \right\}$.
%
However, a simple combination, e.g., averaging or concatenation, of those features may not reflect the spatially-varying property of the generalized SR problem.
%
Therefore, we introduce a multi-scale blending module to combine information from different resolutions effectively.
%
To determine appropriate blending coefficients $w_{\times s}$, image contents play a critical role.
%
For example, low-frequency components are preferred to prevent aliasing and undesirable artifacts for plain regions.
%
On the other hand, high-frequency details matter to accurately represent edges and textures.
%
Therefore, we calculate the content features $\mathbf{C} \in \mathbb{R}^{C \times H' \times W'}$ as follows:
%
\begin{equation}
    \mathbf{C} = \mathcal{C} \paren{ \mathcal{C}_{\times s_0} \paren{ \mathbf{W}_{\times s_0} }, \mathcal{C}_{\times s_1} \paren{ \mathbf{W}_{\times s_1} }, \cdots },
    %\mathbf{C} = \mathcal{C} \paren{ \mathcal{C}_{\times s} \paren{ \mathbf{W}_{\times s} } },
    \label{eq:sampling_contents}
\end{equation}
%
where $\mathcal{C}_{\times s}$ and $\mathcal{C}$ denote learnable scale-specific and global content feature extractors, respectively.


\input{figs/architecture}


Since our SRWarp method handles spatially-varying distortions, an appropriate feature scale may also depend on the local deformation.
%
In other words, providing the degree of transformation at the point may allow our model to adaptively determine the weights of multi-scale representations.
%
Thus, we acquire the scale feature $\mathbf{S} \in \mathbb{R}^{H' \times W'}$ as follows:
%
\begin{equation}
    \mathbf{S} \paren{ x', y' } = -\log{ \lvert \det \paren{ J \paren{ x', y' } } \rvert }.
    \label{eq:sampling_scale}
\end{equation}
%
Physically, the determinant of the Jacobian describes a local magnification factor after transformation.
%
As we adopt backward mapping, we take the reciprocal of the Jacobian determinant and take a natural log for normalization.


We then introduce a sequence of $1 \times 1$ convolutions to a concatenation of the content and scale features.
%
This process determines proper blending weights $w_{\times s}$ for each output position $\paren{ x', y' }$.
%
With the esimated coefficients $w_{\times s}$, the blended features $\mathbf{W}_\text{blend}$ can be represented as follows:
%
\begin{equation}
    \mathbf{W}_\text{blend} = \sum_s {w_{\times s} \odot \mathbf{W}_{\times s}},
    \label{eq:blending}
\end{equation}
%
where $\odot$ is an element-wise multiplication.

\Paragraph{Partial convolution.}
%
Image warping can produce void pixels on the target coordinate when the point is mapped to outside the source image.
%
Since conventional CNNs treat all pixels equally, such regions may negatively affect the model performance around boundaries.
%
To efficiently deal with the problem, we define a 2D binary mask $\mathbf{m}$ as follows:
%
\begin{equation}
    \mathbf{m} \paren{ x', y' } =
    \begin{cases}
        0, & \text{if}\ \paren{ x, y } \text{is outside of}\ \mathbf{F}_{\times{1}} \\
        1, & \text{otherwise}
    \end{cases},
    \label{eq:mask}
\end{equation}
%
where $f_M \paren{ x, y } = \paren{ x', y' }$.
%
To keep consistency between different resolutions, we calculate the mask $\mathbf{m}$ from the $\times 1$ feature $\mathbf{F}_{\times 1}$ and share it across scales.
%
Then, we adopt the partial convolution~\cite{liu2018partialinpainting, liu2018partialpadding} for our content feature extractors $\mathcal{C}$ and $\mathcal{C}_{\times s}$, using the mask to ignore \emph{void} pixels.


\subsection{SRWarp}
\label{ssec:srwarp}
%
Finally, we introduce a reconstruction module $\mathcal{R}$ with 5 residual blocks~\cite{sr_srgan, sr_edsr} to synthesize the output SR result as $\img{SR} = \mathcal{R} \paren{ \textbf{W}_\text{blend} }$.
%
%The module also incorporates the partial convolution for stable training.
%
We combine the SR backbone, AWL, blending, and reconstruction modules to construct the SRWarp model $\mathcal{S}$ as shown in \figref{fig:architecture}.
%
Given a set of training input and target pairs $\paren{ \img{LR}^n, \img{HR}^n }$, we minimize an average $L_1$ loss~\cite{sr_lapsrn, sr_edsr} $\mathcal{L}$ between the reconstructed and ground-truth~(GT) images as follows:
%
\begin{equation}
    \mathcal{L} = \frac{1}{N} \sum_{n = 1}^{N} \frac{ 1 }{ \normzero{ \mathbf{m}} } \normone{ \mathbf{m} \odot \paren{ \mathcal{S} \paren{ \img{LR}^n, f_M } - \img{HR}^n } },
    \label{eq:objective}
\end{equation}
%
where $N = 4$ is the number of samples in a mini-batch, $n$ is a sample index, 0-norm $\normzero{ \cdot }$ represents the number of nonzero values, and $\mathcal{S} \paren{ \img{LR}^{n}, f_M } = \img{SR}^{n}$, respectively.
%
The transform function $f_M$ is shared in a single mini-batch.
%
The binary mask $\mathbf{m}$ from \eqref{eq:mask} prevents backward gradients from being propagated from \emph{void} pixels.
%
The proposed SRWarp model can be trained in an end-to-end manner with the ADAM~\cite{others_adam} optimizer.
%
More specifications about the training data are described in \secref{sec:data_metric}.

==> submission/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}
%
We adopt two different SR networks as a backbone of the multi-scale feature extractor for the proposed SRWarp model.
%
The modified MDSR~\cite{sr_edsr} architecture serves as a smaller baseline, while the RRDB~\cite{sr_esrgan} model with a multi-scale branch (MRDB) provides a larger backbone for improved performance.
%
We describe more detailed training arguments in our supplementary material.
%
We implement our SRWarp method with the PyTorch framework.
%
Codes with an efficient CUDA implementation and dataset will be publicly available to reproduce all provided experiments.


\subsection{Dataset and Metric}
\label{sec:data_metric}
%
In conventional image super-resolution methods, it is very challenging to acquire real-world LR and HR image pairs due to several practical issues such as outdoor scene dynamics, color mismatches, and subpixel misalignments~\cite{sr_realworld, sr_camera, sr_zllz}.
%
Similarly, it is also difficult to collect high-quality image pairs with corresponding transformation matrices in the wild for our generalized SR task.
%
Therefore, we propose the DIV2K-Warping (DIV2KW) dataset by synthesizing LR samples from the existing DIV2K~\cite{data_div2k} dataset to train our SRWarp model in a supervised manner.
%
We first assign 500, 100, and 100 random warping parameters $\left\{ M_{i} \right\}$ for training, validation, and test, respectively.
%
Since we mainly deal with cases where the given image should be enlarged, we formulate each matrix to include random upscaling, sheering, rotation, and projection.
%
We describe more details in our supplementary material.


During the learning phase, we randomly sample square HR patches from 800 images in the DIV2K training dataset and one warping matrix $M_{i}^{-1}$ to construct a ground-truth batch $\img{HR}$.
%
Then, we warp the batch with $M_{i}^{-1}$ to get corresponding LR inputs $\img{LR}$.
%
For efficiency, the largest valid square from the transformed region is cropped to get the input $\img{LR-crop}$.
%
With the transformation matrix $M_{i}$ and LR patches $\img{LR-crop}$, we optimize our warping model to reconstruct the original image $\img{HR}$ as described in \ref{ssec:srwarp}.
%
Figure~\ref{fig:architecture} illustrates the actual training pipeline regarding our SRWarp model.
%
We use 100 images from the DIV2K valid dataset with different transformation parameters following the same pipeline to evaluate our method.


We adopt a traditional PSNR metric on RGB color space for evaluation.
%
However, since the warped images have irregular shapes rather than standard rectangles, we only consider valid pixels in a $H' \times W'$ grid similar to our training objective in \eqref{eq:objective}.
%
The modified PSNR with a binary mask $\mathbf{m}$ (mPSNR) is described as follows:
%
\begin{equation}
    \begin{split}
        \text{mPSNR(dB)} = 10 \log_{10}{ 
            \frac{
                \normzero{ \mathbf{m} }
            }{
                \normtwo{ \mathbf{m} \odot \paren{ \img{SR} - \img{HR} } }
            }
        },
    \end{split}
    \label{eq:mpsnr}
\end{equation}
%
where images are normalized between 0 and 1.


\subsection{Ablation Study}
\label{ssec:ablation}
%
Since the design components of our SRWarp model are orthogonal to each other, we extensively validate their possible combinations in \tabref{tab:baseline}.
%
We use the modified baseline MDSR~\cite{sr_edsr} structure as a backbone by default for lightweight evaluations.
%
We refer to the model with a single-scale SR backbone~\cite{sr_edsr, sr_esrgan} and standard warping layer at the end as a baseline.
%
Sequences of A, M, and R represent the other configurations, e.g., A-R for the one which achieves 31.85dB mPSNR in \tabref{tab:baseline}.
%
More details are described in our supplementary material.


\Paragraph{Adaptive warping layer.}
%
\tabref{tab:baseline} demonstrates that the AWL introduces consistent performance gains by providing spatially-adaptive resampling kernels.
%
\tabref{tab:ablation_warping} extensively compares possible implementations of the AWL in the proposed SRWarp (A-M-R in \tabref{tab:baseline}) model.
%
We first replace the regular resampling grid from M-R in \tabref{tab:baseline} to the spatially-varying representations (Adaptive in \tabref{tab:ablation_warping}) as shown in \figref{fig:example_area_irregular}.
%
However, since the resampling weights $\mathbf{k}$ are not learnable, the formulation does not bring an advantage even the spatially-varying property is considered.
%in \figref{fig:example_area_irregular}.
%
Introducing a kernel estimator to the regular grid (Layer in \tabref{tab:ablation_blending}) yields +0.08dB of mPSNR gain.
%
By combining the spatially-varying coordinates and trainable module, our AWL can further improve the performance to 32.01dB.
%
We note that the adaptive resampling grid does not require any additional parameters and can be calculated efficiently.


\input{tables/sr_ablation}
\input{tables/sr_ablation_detail}


We also analyze two possible variants of the AWL.
%
The AWL-SS configuration in \tabref{tab:ablation_warping} shares the kernel estimator $\mathcal{K}$ across scales and channel dimensions, even with the multi-scale SR backbone.
%
The AWL-MS method in \tabref{tab:ablation_warping} achives a minor performance gain of +0.01dB by utilizing scale-specific modules $\mathcal{K}_{\times s}$ as described in \secref{ssec:ms_warping}.
%
In the proposed SRWarp model, we further estimate the kernels in a depthwise manner, i.e., $C \times k \times k$ weights for each $\paren{ x', y' }$, and achieve an additional +0.05dB improvement in the mPSNR metric.


\input{figs/sr_qualitative}
\input{tables/sr_warp}


\Paragraph{Multi-scale blending.}
%
\tabref{tab:baseline} shows that our multi-scale approach (M) consistently improves the spatially-varying SR performance by a large margin compared to the single-scale counterpart with the baseline EDSR~\cite{sr_edsr} backbone (A-R in \tabref{tab:baseline}).
%
We justify the design of our blending module in \tabref{tab:ablation_blending} by only changing the way to calculate combination coefficients $w_{\times s}$ in \eqref{eq:blending}.
%
Interestingly, simply averaging (Average) the warped features $\mathbf{W}_{\times s}$ produces a better result than concatenating and blending them with a trainable $1 \times 1$ convolutional layer (Concat.).
%
Since the concatenation is a more general formulation, such performance degradation demonstrates that a proper formulation is required for an efficient blending module.
%
We also analyze how content and scale features support the blending module to combine multi-scale representations effectively.
%
If the content information is ignored (w/o $\mathbf{C}$ in \tabref{tab:ablation_blending}), the SRWarp model suffers an mPSNR drop of 0.05dB.
%
Removing the scale term (w/o $\mathbf{S}$ in \tabref{tab:ablation_blending}) also brings a similar degree of performance degradation, justifying the design of our multi-scale blending unit.


\Paragraph{Reconstruction module and Partial convolution.}
%
Since the reconstruction unit $\mathcal{R}$ can further refine output images, it is straightforward that the module brings additional performance gains for all combinations in \tabref{tab:baseline}.
%
We also examine the usefulness of the partial convolution~\cite{liu2018partialinpainting, liu2018partialpadding} in the content feature extractor and reconstruction module.
%
Compared to the previous SR methods, our SRWarp framework is more sensitive to boundary effects due to several reasons.
%
First, image boundaries, i.e., regions between valid and void areas, are not aligned with convolutional kernels and have irregular shapes.
%
Second, since we put irregular-shaped data on a regular 2D grid, numerous void pixels in the warped image negatively affect the following learnable layers.
%
The SRWarp model converges much slower without the partial convolution, and its final performance drops by 0.06dB due to serious boundary effects.


\Paragraph{Backbone architecture.}
%
The last two rows of \tabref{tab:baseline} compare how different backbone architectures affect the performance of the SRWarp method.
%
Using the larger MRDB network with 17.1M parameters brings a significant PSNR gain of +0.27dB compared to the MDSR backbone with 1.7M parameters, showing that our SRWarp can benefit from more computational resources.


\input{tables/sr_arbitrary}


\subsection{Comparison with the Other Methods}
%
We compare the proposed SRWarp with existing warping methods.
%
Since our approach is the first attempt to extend the concept of the SR to general image transformation, we note that it is difficult to provide an exact comparison to the other methods.
%
First, we adopt a conventional interpolation-based warping algorithm from the OpenCV framework~\cite{opencv_library}.
%
We use {\fontfamily{qcr}\selectfont cv2.WarpPerspective} function with a bicubic kernel to synthesize output warped images.
%
For alternative methods, we combine state-of-the-art SR models and the traditional warping operation.
%
Since the given LR images are supersampled before interpolation, high-quality warping results can be synthesized straightforwardly.


\tabref{tab:comp} provides quantitative comparison between aforementioned methods.
%
For fair comparison, we adopt the DIV2KW$_\text{Test}$ dataset rather than the validation split used in \secref{ssec:ablation}.
%
Compared to the traditional warping algorithm (\cv{cv2}), using the SR methods provides significant improvements with the mPSNR gain of at least +2.41dB.
%
Higher-scale SR models tend to produce better results, showing that the fine-grained supersampling is essential for the following transformation process.
%
The proposed SRWarp with the MRDB backbone further outperforms the other SR-based formulations by a large margin.
%
\figref{fig:qualitative} illustrates that our approach reconstructs much sharper images with less aliasing, demonstrating the effectiveness of the adaptive warping layer and multi-scale blending.


\subsection{Arbitrary-scale SR}
%
Our SRWarp provides a generalization of the conventional SR models defined on scaling matrices in \eqref{eq:scale_matrix} only.
%
To justify that the proposed framework is compatible with existing formulations, we evaluate our method on the regular SR task of arbitrary scaling factors.
%
We train the SRWarp model with RRDB~\cite{sr_esrgan} backbone on fractional-scale DIV2K dataset~\cite{sr_meta} and evaluate it following Hu~\etal~\cite{sr_meta}.
%
While the input transformation of the SRWarp is constrained to \eqref{eq:scale_matrix}, the other configurations are kept fixed.
%
\tabref{tab:fractional} shows an average PSNR of the luminance (Y) channel between SR results and ground-truth images on B100~\cite{data_bsd200} dataset.
%
We note that the SRCNN~\cite{sr_srcnn} and VDSR~\cite{sr_vdsr} methods first resize the input image to an arbitrary target resolution before take it into the network.
%
Compared to the meta-upscale module (Meta-EDSR and Meta-RDN), our adaptive warping layer and multi-scale blending provide a more efficient and generalized model for the arbitrary-scale SR task.


\input{figs/sr_functional}
\subsection{Over the Homographic Transformation}
%
While we mainly focus on projective mappings to formulate our SRWarp model, it is also possible to apply the proposed framework to arbitrary functional transforms.
%
Given a backward mapping equation $f^{-1}_{M} \paren{ x', y' } = \paren{ x, y }$, it is straightforward to extend the proposed method without \emph{any} modification.
%
While the proposed SRWarp model is trained on homographic transformation only, the adaptive warping layer and multi-scale blending help the method be generalized well on unseen deformations.
%
\figref{fig:functional} compares our results on various functional transforms against the combination of the RRDB~\cite{sr_esrgan} supersampler and traditional bicubic interpolation.
%
Our SRWarp model can provide more flexibility and diversity in general image editing tasks by reconstructing sharper edges with less aliasing.

==> submission/5_conclusion.tex <==
\section{Conclusion}
%
In this paper, we propose a generalization of the conventional SR tasks under image transformation for the first time.
%
Unlike previous approaches, our SRWarp framework deals with the spatially-varying upsampling task when arbitrary resolutions and shapes are required to the output image.
%
We also provide extensive ablation studies on the proposed method to validate the contributions of several novel components, e.g., adaptive warping layer and multi-scale blending, in our design.
%
The visual comparison demonstrates why the SRWarp model is required for image warping and validates the advantage of the proposed method.
